Statistical dependence: Beyond Pearson's $\rho$

Pearson's $\rho$ is the most used measure of statistical dependence. It gives a complete characterization of dependence in the Gaussian case, and it also works well in some non-Gaussian situations. It is well known, however, that it has a number of shortcomings; in particular for heavy tailed distributions and in nonlinear situations, where it may produce misleading, and even disastrous results. In recent years a number of alternatives have been proposed. In this paper, we will survey these developments, especially results obtained in the last couple of decades. Among measures discussed are the copula, distribution-based measures, the distance covariance, the HSIC measure popular in machine learning, and finally the local Gaussian correlation, which is a local version of Pearson's $\rho$. Throughout we put the emphasis on conceptual developments and a comparison of these. We point out relevant references to technical details as well as comparative empirical and simulated experiments. There is a broad selection of references under each topic treated.

==> preamble_arxiv.tex <==
\newcommand{\Cov}{\textrm{Cov}}
\newcommand{\E}{\textrm{E}}
\newcommand{\Var}{\textrm{Var}} 
\newcommand{\di}{\,\textrm{d}}
\newcommand{\Corr}{\textrm{Corr}} 

\usepackage{graphicx}
\usepackage{subfig}
\usepackage{bm}


